Understanding Missingness in Time-series Electronic Health Records for Individualized Representation

With the widespread of machine learning models for healthcare applications, there is increased interest in building applications for personalized medicine. Despite the plethora of proposed research for personalized medicine, very few focus on representing missingness and learning from the missingness patterns in time-series Electronic Health Records (EHR) data. The lack of focus on missingness representation in an individualized way limits the full utilization of machine learning applications towards true personalization. In this brief communication, we highlight new insights into patterns of missingness with real-world examples and implications of missingness in EHRs. The insights in this work aim to bridge the gap between theoretical assumptions and practical observations in real-world EHRs. We hope this work will open new doors for exploring directions for better representation in predictive modelling for true personalization.

==> main2.tex <==
% \documentclass[fleqn,10pt]{wlscirep}
% \usepackage[utf8]{inputenc}
% \usepackage[T1]{fontenc}
% \usepackage{bm}
% \usepackage{natbib}
% \title{What's missing in AI for healthcare models? A new perspective on representing missingness in Electronic Health Records.
% }
% \usepackage{comment}  % PW added

% %\title{Individualized Generation of Time-series Electronic Health Records for Personalised Care}
% % \title{Generation of Personalised Longitudinal Electronic Health Records for Medical Applications}

% % Use letters for affiliations, numbers to show equal authorship (if applicable) and to indicate the corresponding author
% \author[1,*]{Ghadeer O. Ghosheh}
% \author[2]{Jin Li}
% \author[1]{Tingting Zhu}

% \affil[1]{University of Oxford}

% \affil[2]{Nanjing University of Information Science \& Technology (NUIST)}


% \affil[*]{Correspondence: ghadeer.ghosheh@eng.ox.ac.uk}
% \begin{comment}
% \begin{abstract}

% \end{abstract}
% \end{comment}

% \begin{document}

% \maketitle
% \thispagestyle{empty}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % (1) wide-spread of ML models, yet there's limited focus on missingness representation in building such models. 
% %(2) EHRs such as MIMIC can be as high as 80% missing
% %(3) there's a gap that needs to be filled
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% With the increased adoption of electronic health records (EHRs), many machine-learning for healthcare applications have demonstrated great promise~\citep{xiao2018opportunities,shamout2020machine}. 
% Ranging from diagnostic models to models that predict clinical deterioration and treatment effects, machine learning models have shown improved performance in learning representations for data collected over time and using the learned representations for a wide range of tasks when compared to classical statistical models.  However, EHRs tend to be highly missing and irregularly sampled~\citep{madden2016missing} with missingness reaching up to 80\% in commonly used intensive care unit datasets such as MIMIC~\citep{johnson2016mimic} and eICU~\citep{pollard2018eicu}. These numbers suggest a pressing need for learning a proper representation and analysis of the nature of missingness to better serve the target application without performance deterioration at the deployment stage.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % (1) Missingness has been studied from theoretical angles 
% % (2) introduce types of missingness
% %(3) Notwithstanding the importance of such works and many deep learning works, theoretical assumptions for MCAR are hard to prove and not suitable for real-world applications
% % (4) why missingness occurs in healthcare, ex: cost, patient deterioration, bias....etc 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Most works discussing missingness in data focus on theoretical assumptions that classify missingness as one of the following classes, missing completely at random (MCAR), missing at random (MAR), and not missing at random (NMAR)~\cite{little2019statistical}. In the case of MCAR, it is assumed that the missingness in the data is not related to either the observed or unobserved data~\cite{mack2022types}. On the other hand, in the case of MAR, the missingness is dependent on the observed data only, compared to MNAR where the nature of missingness is systematically related and depends on unobserved data~\cite{mack2022types}.  Notwithstanding the importance of theoretical works and the highly reported performance of deep learning models for imputation tasks~\citep{yoon2018gain,cao2018brits,fortuin2020gp}, most works focus on MCAR settings which imposes strong assumptions on the nature of data missingness. However, in healthcare settings missingness in many cases is informative and depends on factors that might or might not be captured in the data~\citep{scheffer2002dealing}, limiting many of the utility of the proposed work in real-world healthcare applications.
% %Such strong assumptions regarding the nature of missingness limit their potential in real healthcare applications, where missingness can be informative and reflect individual-level difference.
% Understanding the implications of missingness in EHRs requires understanding various potential reasons for missingness in real-world healthcare.  Missingness in the healthcare domain can occur due to various reasons such as recording errors and machine failure, irregular sampling and inconsistent medical visits~\citep{kreindler2006effects}, or even high-cost and dangerous to acquire information such as invasive or radiology procedures~\citep{bulas2013benefits,kim2017dangers}. In addition, the measurement frequency could also be related to factors such as patient severity and  deterioration~\citep{agniel2018biases,ghosheh2022review}, lack of medical need~\citep{duff2019frequency},  bias and quality of care~\citep{weber2021gender,wells2013strategies}, which could vary from one patient to another, indicating the importance of representing the individualized missingness in personalized medicine models. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % (1) current literature on ML focuses on observed data and neglects to represent missingness
% %(2) recent few works used the binary mask as input found them to be equally informative to the real-observed values indicating the value of missingness in various ML for healthcare tasks
% %(3) Despite importance of masks "binary", there are other patterns of missingness in time-series data that are not well studied and we shed light on them with examples from real settings 
% % (4) feature-wise and sample-wise missingness

% % (5) limitations of mean imputation ...distribution wrong 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The current literature on personalized medicine proposes methods that only focus on the observed data~\citep{chen2019deep,wang2016learning} and often overlook the "individualized" and informative nature of missingness. Recent ML for healthcare works have shown that the utilization of binary missingness masks indicating the presence of observations as input features to prediction models results in equivalent performance to those built on real values of clinical features~\citep{sharafoddini2019new,che2018recurrent}, indicating the predictive value of missingness patterns. However, despite the utility and predictiveness of the binary missingness masks, they are simplistic and lack indications of the patterns and frequencies of individual-level missingness for each patient. 


% Here, we highlight new insights into patterns of missingness in EHRs, which require a new perspective on representing missingness beyond binary masks.
% In longitudinal or time-series EHRs,
% % the frequency of measurement of a variable over time steps of a specific variable is indicated by several factors including patient severity, patient adherence and frequencies of visits. 
% the frequency of measurement of a variable over time is often indicative of the patient's underlying state.  Some lab values are only measured for severe patients to rule in or rule out clinical complications, so a single measurement of a feature is enough to indicate the patient's case.  For example, cardiac Troponins, sensitive biomarkers of myocardial injury (MI), are not ordered for every patient in the ICU but are rather ordered for patients suspected of having a cardiac-related diagnosis or complication ~\citep{daubert2010utility}. In the same intuition, a missing measurement of cardiac Troponins can indicate that the patient is not suspected of developing such complications, as the clinical guidelines only recommend this measurement for diagnosing myocardial injury~\citep{collinson2022troponin}.  We refer to the missingness of observations of a variable across a patient record as feature-wise missingness. 


% Understanding the difference between general missingness in a patient record and feature-wise missingness for some variables is crucial to understanding the implications of imputing the missing values. For example, filling the missing values for cardiac troponin for healthy patients all of which have feature-wise missingness,  by the population mean will result in an imputation value above the healthy range as all the available measurements are for patients suspected of having MI and therefore result in flawed representation and data distribution. Due to the limitations of such simple imputation techniques in handling individualized patterns in missingness, we believe that new approaches to representing missingness in predictive models can help in generating high-quality imputations and building high-performance and robust predictive models.  In our recent work in Individualized GeNeration of Imputations in Time-series Electronic health records (IGNITE), we present a new frequency-based Individualized Missingness Mask (IMM) where the binary mask is transformed into an individual-level mask reflective of the frequency of measurement of features across time. The power of the IMM opens new doors for exploring directions for better missingness representation in predictive modelling.  As we believe that the imputation and representing missingness in the EHRs is beyond a preprocessing step, the field is not complete without proper handling and representation of missingness in the data. 


% % but rather a fundamental step that would impact the 

% % AI for healthcare models is not complete without proper handling of missingness in data.  




% % 2 percent missingness in a longitudinal record composed of 10 variables, it is different when the patient has 25\% of each variable missing across time-steps, vs 8 variables completely measured across all time-steps and 2 variables never collected for the patient. In the former case, missingness might be related to error, random chance. The two variables never measured might mean 


% % However, this kind of feature-level missingness, can not be represented in the traditional binary missingness masks. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% % The Correspondence section provides a forum for discussion or to present a point of view on issues that are of interest to the readership of Nature Medicine. Correspondences should not contain new research data, nor should serve as a venue for technical comments on peer-reviewed research papers, which would be considered Matters Arising.

% % Correspondences are initially screened for general interest, and may be returned to the authors if the topic, angle or content is deemed not to be of high interest to the journal’s readership or when the topic has already been covered in other pieces. Nature Medicine receives a very high volume of correspondence and the editorial team reserves the right to return submissions to authors without further feedback. After screening, correspondences are edited for concision and clarity, and additional changes may be requested from the authors. 

% % Format

% % Main text – up to 1,000 words.
% % Display items – up to 2 items.
% % References – up to 10 references. Article titles are omitted from the reference list.
% % Correspondence may be peer-reviewed at the editors’ discretion. 

% \bibliography{sample}

% \end{document}
